Wisdom of Instruction-Tuned Language Model Crowds. Exploring Model Label Variation

Large Language Models (LLMs) exhibit remarkable text classification capabilities, excelling in zero- and few-shot learning (ZSL and FSL) scenarios. However, since they are trained on different datasets, performance varies widely across tasks between those models. Recent studies emphasize the importance of considering human label variation in data annotation. However, how this human label variation also applies to LLMs remains unexplored. Given this likely model specialization, we ask: Do aggregate LLM labels improve over individual models (as for human annotators)? We evaluate four recent instruction-tuned LLMs as annotators on five subjective tasks across four languages. We use ZSL and FSL setups and label aggregation from human annotation. Aggregations are indeed substantially better than any individual model, benefiting from specialization in diverse tasks or languages. Surprisingly, FSL does not surpass ZSL, as it depends on the quality of the selected examples. However, there seems to be no good information-theoretical strategy to select those. We find that no LLM method rivals even simple supervised models. We also discuss the tradeoffs in accuracy, cost, and moral/ethical considerations between LLM and human annotation.

==> competence_hateval.tex <==
\begin{table*}[htb!]
\small
\centering
\setlength{\tabcolsep}{5pt}
\begin{tabular}{ccccccc}
\toprule
\multicolumn{2}{c}{\textbf{Task/Language}} & \textbf{T0} & \textbf{Flan-T5} & \textbf{Flan-UL2} & \textbf{Tk-Instruct} & \textbf{Alpaca}  \\
\midrule
\multirow{3}{*}{SA} 
& EN & 0.784 & \textbf{0.921} & 0.897 & 0.789 & 0.788 \\
& DE & 0.758 & \textbf{0.902} & 0.789 & 0.751 & 0.704 \\
& FR & \textbf{0.884} &	0.824 & 0.773 & 0.795 & 0.681 \\
\midrule
\multirow{3}{*}{AC-Gender} 
& EN & 0.313 & 0.615 & \textbf{0.711} & 0.453 & 0.070 \\
& DE & 0.149 & 0.270 & \textbf{0.362} & 0.273 & 0.108 \\
& FR & \textbf{0.693} & 0.595 & 0.611 & 0.094 & 0.177 \\
\midrule
\multirow{3}{*}{AC-Age} 
& EN & 0.243 & 0.146 & \textbf{0.326} & 0.085 & 0.145 \\
& DE & 0.298 & 0.039 & \textbf{0.412} & 0.014 & 0.344 \\
& FR & 0.060 & \textbf{0.689} & 0.380 & 0.017 & 0.261 
\\
\midrule
\multirow{3}{*}{TD} 
& EN & 0.388 & 0.736 & \textbf{0.932} & 0.511 & 0.025 \\
& DE & 0.658 & \textbf{0.797} & 0.740 & 0.714 & 0.060 \\
& FR & 0.210 & \textbf{0.556 }& 0.326 & 0.492 & 0 \\
\midrule
\midrule
\multirow{3}{*}{Mean} 
& EN & 0.432 & 0.605 & \textbf{0.717} & 0.460 & 0.257 \\
& DE & 0.466 & 0.502 & \textbf{0.576} & 0.438 & 0.304\\
& FR & 0.411 & \textbf{0.644} & 0.483 & 0.378 & 0.224 \\
\bottomrule
\midrule
\multirow{2}{*}{HS} 
& EN & 0.358 & \textbf{0.912} & 0.327 & 0.404 & 0.050
 \\
& ES & \textbf{0.465} & 0.212 & 0.131 & 0.099 & 0.009
\\
\bottomrule

\end{tabular}
\caption{MACE competence scores of each LLM across tasks and languages on the Trustpilot and HatEval datasets.}
\label{tab:tab_competence_trustpilot}
\end{table*}

==> dataset.tex <==
\begin{table}[htb!]
\centering
\small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{ll}
\toprule
\textbf{Task} & \textbf{Label}      \\ \midrule
AC & Gender: \textit{male}, \textit{female}         \\ 
& Age: \textit{under 35}, \textit{above 45}         \\ \midrule
SA & \textit{negative}, \textit{neutral}, \textit{positive}    \\ \midrule
TD & Five distinct topic categories \\
\midrule
HS & \textit{hate-speech}, \textit{non-hate speech} \\ 
\bottomrule
\end{tabular}
\caption{Classification tasks considered in our study.}\label{table:tasks}
\label{tab:text-classification}
\end{table}


==> fs_results.tex <==
\begin{table*}[t]
  \small
  \centering
    \setlength{\tabcolsep}{3pt}
    \begin{tabular}{ll|cccc|cc}
      \toprule
      \multicolumn{2}{c|}{\textbf{Task/Strategy (FS)}} & \textbf{T0} & \textbf{Flan-T5} & \textbf{Flan-UL2} & \textbf{Tk-Instruct} & \textbf{Majority} & \textbf{MACE} \\
      \midrule
      \multirow{3}{*}{SA} 
       & $\downarrow$ E & 0.168 & 0.530 & 0.496 & 0.167 & 0.491 & 0.532 \\
       & $\uparrow$ E & \textbf{0.337} & \textbf{0.556} & 0.496 & \textbf{0.594} & \textbf{0.527} & \textbf{0.546} \\
       & Random & 0.166 & 0.167 & 0.496 & 0.167 & 0.496 & 0.496\\
      \midrule
      \multirow{3}{*}{AC-Gender} 
      & $\downarrow$ E & \textbf{0.513} & \textbf{0.604} & \textbf{0.625} & 0.355 & 0.587 & 0.621 \\
      & $\uparrow$ E & 0.335 & 0.540 & 0.619 & 0.338 & 0.578 & 0.586 \\
      & Random & 0.474 & 0.580 & 0.631 & \textbf{0.346} & 0.529 & \textbf{0.631} \\
      \midrule
      \multirow{3}{*}{AC-Age}
       & $\downarrow$ E & 0.336 & 0.409 & \textbf{0.527} & 0.332 & \textbf{0.544} & \textbf{0.527} \\
       & $\uparrow$ E & 0.336 & \textbf{0.489} & 0.396 & 0.332 & 0.537 & 0.489 \\
       & Random & 0.336 & 0.383 & 0.515 & 0.332 & 0.536 & 0.515 \\
      \midrule
      \multirow{3}{*}{TD}
       & $\downarrow$ E & 0.057 & 0.063 & 0.604 & 0.063 & 0.161 & 0.604 \\
       & $\uparrow$ E & \textbf{0.085} & 0.057 & 0.599 & 0.057 & 0.146 & 0.599 \\
       & Random & 0.085 & \textbf{0.067} & \textbf{0.605} & \textbf{0.085} & \textbf{0.167} & \textbf{0.605}  \\
       \midrule
       \midrule
       \multirow{3}{*}{Mean}
       & $\downarrow$ E & 0.269 & 0.401 & \textbf{0.563} & 0.229 & 0.446 & 0.571 \\
       & $\uparrow$ E & \textbf{0.273} & \textbf{0.411} & 0.528 & \textbf{0.330} & \textbf{0.447} &	0.555 \\
       & random & 0.265 &	0.299 &	0.562 &	0.232 &	0.432 &	\textbf{0.562} \\
      \bottomrule
    \end{tabular}
  \caption{Few-shot Macro-F1 results obtained by the LLMs on the English Trustpilot tasks along with the aggregation methods.
  FSL strategies: Low Entropy ($\downarrow$ E), Max Entropy ($\uparrow$ E), and Random.
  Results in bold show the best few-shot strategy performance by LLM.}
  \label{tab:fs_results}
\end{table*}


==> results_hateval.tex <==
\begin{table*}[ht!]
\small
\centering
\resizebox{\textwidth}{!}{%
\setlength{\tabcolsep}{4pt}
\begin{tabular}{cc|ccccc|cc|cc}
\multicolumn{2}{c|}{} & \multicolumn{5}{c|}{\textbf{Models}} & \multicolumn{2}{c|}{\textbf{Baselines}} & \multicolumn{2}{c}{\textbf{Aggregate}}\\
\toprule
\multicolumn{2}{c|}{\textbf{Task/Lang.}} & \textbf{mT0} & \textbf{Flan-T5} & \textbf{Flan-UL2} & \textbf{Tk-Instruct} & \textbf{Alpaca} & \textbf{Most Freq.} &  \textbf{Random} &  \textbf{Majority} & \textbf{MACE} \\
\midrule
\multirow{2}{*}{HS} 
& EN & 0.621$^{\star}$ & 0.726$^{\star}$ & 0.670$^{\star}$ & 0.579$^{\star}$ & 0.428 & 0.367 & 0.490 & \textbf{0.732}$^{\star}$  & 0.726$^{\star}$  
\\
& ES & 0.601$^{\star}$ & 0.532$^{\star}$ & 0.519 & 0.449 & 0.394 & 0.370 & 0.492 & 0.476 & \textbf{0.603}$^{\star}$
\\
\bottomrule
\end{tabular}
}
\caption{Macro-F1 results obtained by the LLMs on the HatEval dataset, the baselines and the aggregation methods. Best result per language and task is shown in bold. Significant improvement over Random baseline ($^{\star}: p \leq 0.01$) with bootstrap sampling. For  non-English languages, we use the multilingual mT0 model.}\label{tab:results_hateval}
\end{table*}
